MaTIC: a Mathematical Theory of Inferential Communication

The arrival of Immersive Virtual and Augmented Reality hardware to the consumer market suggests seamless multi-modal communication between human participants and autonomous interactive characters is an achievable goal in the near future. This possibility is further reinforced by the rapid improvements in the automated analysis of speech, facial expressions and body language, as well as improvements in character animation and speech synthesis techniques. However, we do not have a formal theory that allows us to compare, on one side, interactive social scenarios among human users and autonomous virtual characters and, on the other side, pragmatic inference mechanisms as they occur in non-mediated communication. Grices' and Sperbers' model of inferential communication does explain the nature of everyday communication through cognitive mechanisms that support spontaneous inferences performed in pragmatic communication. However, such a theory is not based on a mathematical framework with a precision comparable to classical information theory. To address this gap, in this article we introduce a Mathematical Theory of Inferential Communication (MaTIC). MaTIC formalises some assumptions of inferential communication, it explores its theoretical consequences and outlines the practical steps needed to use it in different application scenarios.

==> MaTIC - Inferential Communication Theory - OUT/removed.tex <==



We can do so with the following logical operation, which applies over chains of events:
\begin{definition}
    \textbf{AND} ($\wedge$) is a function defined on the \emph{possibility} domain, and it has the following properties:
    \begin{enumerate}
        \item     The function must be monotonous, but not necessarily be linear, or even continuous.  This means that if one input variable increases (while everything else being equal), then the output should stay  the same or increase, but not decrease.
        \item The output should not be bigger than any of its inputs
    \end{enumerate}

\end{definition}
        
 A typical example of a mathematical function with such properties is the minimum operation. The boolean AND operator also satisfies these properties, if the inputs are binary.  Conversely, for an agent to determine whether an event must be triggered, from a set of possible causes, we may use the following operator:
        
        
\begin{definition}
        \textbf{OR} ($\vee$) is defined on the \emph{necessity} 
        domain, and it has the following properties:
    \begin{enumerate}
        \item     The function must be monotonous, but not necessarily be linear, or even continuous.  This means that if one input variable increases (while everything else being equal), then the output should stay  the same or increase, but not decrease.
        \item The output should not be smaller than any of its inputs
    \end{enumerate}

\end{definition}
  A typical example of a mathematical function with such properties is the maximum operation. The boolean OR operator also satisfies these properties, if the inputs are binary. 
  
    In general, the  `$\wedge$' and `$\vee$' functions apply over chains of events like $a.b.c$, and therefore they are not commutative. Intuitively, the proposition ‘\textbf{He gets angry AND she cries}’ does not imply the same as ‘\textbf{She cries AND he gets angry}’. 
  Since we are referring to events, the meaning of a formula like ‘$a\wedge b$’  is better captured if instead of reading as \emph{a and b} one reads it as \emph{a and then b}.
The causal relations suggested by these sentences are not the same, and they do not suggest the same meaning. Therefore, quantifying the likeliness that one of these sequences occurred or will occur does not say anything about the likeliness of the other occurring. 
  On the other side, the `$\wedge$' and `$\vee$' operators do satisfy the usual associative properties. For example, ‘$(a \wedge b) \wedge c$’ is equivalent to ‘$a \wedge (b \wedge c)$’.
  


The distributive property therefore applies between `$\vee$' and `$\Rightarrow$':  ‘$(a \vee b) \Rightarrow c$’ is equivalent to ‘$(a \Rightarrow c) \vee (b \Rightarrow c)$’.
%through the chains of causal relations  when the communicative sequence $S$ is instantiated in a set of  agents exchanging intentional actions. 


DISCUSSION on causality:





A major conundrum we have faced is how to define \emph{Cause} if  some of these causal relations need to be \emph{implicatures}. The problem is that such a definition needs to work  within a dynamic and non-linear environment, and triggered by the beliefs of agents perceiving and acting in such environments. If we look into complex systems theory as applied in statistical physics or in economics, there is no easy way to  define causality. \cite{auyang1999foundations}, in page 314, writes:


\begin{quote}The best way to establish a temporal direction is to base it on a general concept, so that we need not go into the substantive details of various processes. The most likely candidate for such a general concept is causality. If we can find a notion of causation that is independent of the concept of time, then we can establish a general temporal direction by identifying it with the direction of causation. The task is not easy [...]. Philosophers do not succeed in finding a time-independent notion of causation. \end{quote}

Therefore, whatever formalism we use to define a cause, we will need to show it applies to implicatures, but also to traditional, rather physical, causes. And, of course, traditional logic implications. Is our formalism general enough to encompass these three uses of causality? Further work should spell out more explicitly the relation between this model and the different ways  causal inferences are formalized (propositional logic, Bayesian inference, Structural Equation Modelling, etc.) 



removed

from discussion:




idea of mathematical representations as a set of conceptual metaphors grounded in embodied cognitive mechanisms, much like \cite{lakoff2000mc}. Further work should be done to confirm the detail of how it is built with  rigorous mathematical foundations, but yet in an accessible pedagogic way, as is the case with typical textbooks focused on ZFC set theory, which assume implicitly the thesis of mathematical realism: that sets are entities that exist, in and of themselves, and that the entire universe of discourse can be derived from that fundamental assumption, and technical axioms.




A benefit of this formalism is that it provides a set of principles,% logic,
driven by explicit assumptions, which can be used to compare different inference methods and different computational models of human inference. A second benefit is that it allows formalising inferential communication \emph{in general}, both for human participants and for computational entities embodied in virtual characters.
A third benefit is that it does not contradict previous formalisms related to inference and communication: introducing additional restrictions to the assumptions, the formalism results in different formal frameworks, such as classical information theory, or even classical propositional logic. 
%TO DELETE, FROM WIKIPEDIA, JUST TO RETHINK The addressee uses the information contained in the utterance together with his expectations about its relevance, his real-world knowledge, as well as sensory input, to infer conclusions about what the communicator wanted to convey. Typically, more conclusions can be drawn if the utterance contains information that is related to what the addressee already knows or believes. In this inference process, the "literal meaning" of the utterance is just one piece of evidence among others.[2]Sperber and Wilson sum up these properties of verbal communication by calling it ostensive-inferential communication.[3] it is characterised by two layers of intention on part of the communicator:[4]a. The informative intention: The intention to inform an audience of something (to communicate a certain content).b. The communicative intention: The intention to inform the audience of one's informative intention (to draw the audience's attention to one's informative intention).
This suggests this formalism could be used as a common framework to compare different  reasoning styles that may be used in inferential communication, including formal reasoning mechanisms such as Bayesian inference, classical propositional reasoning, or computational heuristics often built ad hoc for conversational agents. 


